ConceptEVA: Concept-Based Interactive Exploration and Customization of Document Summaries

With the most advanced natural language processing and artificial intelligence approaches, effective summarization of long and multi-topic documents -- such as academic papers -- for readers from different domains still remains a challenge. To address this, we introduce ConceptEVA, a mixed-initiative approach to generate, evaluate, and customize summaries for long and multi-topic documents. ConceptEVA incorporates a custom multi-task longformer encoder decoder to summarize longer documents. Interactive visualizations of document concepts as a network reflecting both semantic relatedness and co-occurrence help users focus on concepts of interest. The user can select these concepts and automatically update the summary to emphasize them. We present two iterations of ConceptEVA evaluated through an expert review and a within-subjects study. We find that participants' satisfaction with customized summaries through ConceptEVA is higher than their own manually-generated summary, while incorporating critique into the summaries proved challenging. Based on our findings, we make recommendations for designing summarization systems incorporating mixed-initiative interactions.

==> abstract.tex <==
abstract 

% Insert line break before ccsdesc for EuroVis template
\\


==> sections/XX-use_cases.tex <==
In this section, we illustrate the use of our approach for summary evaluation and customization in one use case scenario.
This scenario involves Alice, a Ph.D. student in computer science, who is building her knowledge base in infovis by collecting and reading prominent articles in the area.
She finds a paper by Munzner~\cite{munzner2009nested} titled \textit{A Nested Model for Visualization Design and Validation}, which she loads into \techname.

% starts to research in information visualization by collecting and reading some distinguished papers in this area, among which there is one entitled \textit{A Nested Model for Visualization Design and Validation}~\cite{munzner2009nested}.
% The content and the original abstract of the paper look a bit complex to her, so she decides to use \techname to make a better sense of the paper.

\noindent
\textbf{Summary Evaluation.} 
After loading the paper into \techname, an auto-generated summary of the paper content is displayed in the summary view (Fig.~\ref{fig:interface}-3).
\techname\ shows the ROUGE score of the summary to be 0.25, indicating that the summary is somewhat different from the original abstract of this paper.
Alice decides to compare her exploration of the summary by examining the concepts from the paper that are \textit{not} in the summary.
She sets the ConceptView to display concepts by frequency, and examines dominant concepts that are not yet included in the summary (Fig.~\ref{fig:interface}-2).
Among these concepts, she chooses \textit{``algorithm''}, \textit{``abstraction''}, and \textit{``data compression''} as concepts to include, and regenerates the summary, replacing the previous one.
Going through the new summary, Alice sees that the dominant concepts are highly related to the topic of ``four levels of a nested model''.
% \skc{@Xiaoyu: how can Alice see this topic?} \xz{@Senthil: She can see it from summary content. There are several bullet points about this topic}
Skimming through the sections in the document view on the left (Fig.~\ref{fig:interface}-1), Alice interprets the topic of the nested model as critical, which the initial summary had not sufficiently addressed.

% Therefore, Alice decides to start her exploration by finding the missing concepts in this summary.
% When she looks at the concepts in ConceptView (Fig.~\ref{fig:interface}-2), she noticed that over half of the concepts are excluded from this summary, including some dominant concepts according to their frequency, such as ``algorithm'', ``abstraction'' and ``data compression''  (Fig.~\ref{fig:interface}).
% After selecting the dominant missing concepts and generating a summary about them, Alice found that they are highly related to the topic of ``four levels of a nested model''.
% Given that ``nested model'' also appears in the paper title and the title of a section (Fig.~\ref{fig:interface}-1), Alices takes it as a critical topic which the provided summary hasn't sufficiently addressed.
% According to the quantitative score and the qualitative observations she has collected so far, Alice concludes that the quality of the abstract is not satisfying enough, especially concerning the critical topic ``nested model''.

\noindent
\textbf{Summary Customization.} 
Based on the above observations, Alice decides to customize a summary that reveals more information about the topic ``nested model''.
% She first tries to generate such summary simply by selecting the section entitled ``nested model'', but the result is not satisfying enough.
She chooses the PCA algorithm to project the concepts and examines the neighbors of the concepts \textit{algorithm}, \textit{abstraction}, and \textit{data compression}.
She reasons that the exclusion of \textit{data compression} is acceptable as its related concepts and neighbors in ConceptView---\textit{data} and \textit{data type}---are already included in the summary.
She then looks at \textit{algorithm} and finds its neighboring concepts also excluded from the summary.
She decides to add \textit{algorithm} to include in the summary to be generated.
When checking the distribution histogram from the concept \textit{glyph} and section headers, she finds that the concept \textit{information visualization} appears only once in the summary in relation to the term ``visualization designer'' even though it appears prominently throughout the source document.
She finds this to be a misrepresentation of the concept, and so adds it to the list to be included in the summary to be generated.
The iterates through these three concepts once again, this time using the ``focus on'' function to examine and fine-tune the inclusion of related concepts.
She reads through the new summary generated and sees that it better represents the information about the ``nested model''. She then goes on to edit the generated list of sentences to flow better into a paragraph that she then incorporates into her notes.

% She projects the concept with the ``PCA'' algorithm and looks at the neighbors of the excluded dominant concepts mentioned above, and reasons that the missing of ``data compression'' is acceptable because its neighbors, concepts ``data'' and ``data type'', are already included in the summary, covering similar semantic information to ``data compression''.
% However, the missing ``algorithm'' is a more severe problem because none of its neighbors are included in the summary.
% Therefore, she decides to only add ``algorithm'' into her concept list for summary customization.
% Then she turns to examine the dominant concepts appearing both in the original document and the summary.
% When looking at the concept \textit{glyph} of ``information visualization'', she found it appears uniformly across the entire paper, but only appears once at the beginning of the summary.
% She thus uses the coordinated highlighting and the histogram overlaid on top of the section headers to rapidly locate the context of this concept and scan through it.
% She found this concept covers rich semantics in the original document but only refers to ``visualization designer'' in the summary.
% Therefore, she also adds this concept into her concept list because though appearing once in the summary, this concept is also misrepresented.
% Finally, she uses the ``focus on'' function to add more related concepts about this topic \xz{such as..} and starts the customized summary generation.
% This time, she feels the new summary provides enough information about the ``nested model'' and moves on to merge the summarized bullet points into a paragraph that she could save into her reading notebook.

\begin{figure*}
  \centering
  \includegraphics[width=0.95\linewidth]{figures/use_case.png}
  \caption{
  Snapshots of the \techname\ interface showing actions performed in Sec.~\ref{sec:use-case-scenario}.
  The central ConceptView is shown on the left, showing concepts that are included (dark gray box \& arrow) in the summary, concepts that are excluded (light gray box \& arrow) from the summary, and excluded concepts that are selected to be included (orange box \& arrow) in a customized version of the summary.
  Certain excluded concepts, such as \textit{``data compression''} are well-represented by neighbouring concepts that are included in the summary, and thus may not merit inclusion.
  Other concepts like ``algorithm'' may be excluded along with its neighbours, while yet other concepts (see ``information visualization'') might be misrepresented on closer examination of the summary and the document.
  These can be deemed necessary to include in the summary.
  The auto-generated summary that incorporates the new concepts is shown on the right.
  For more details see Sec.~\ref{sec:use-case-scenario}.
 }
 \label{fig:use_case}
\end{figure*}


==> sections/approach.tex <==
The research plan goes here.

Suggestion: Define an "importance metric" to rank the concepts retrieved from DBPedia that feature in the summary. (what about concepts that are in the document but not in the summary?)
If the importance metric is something new that we propose, we need to incorporate the metric's performance into the user study (or devise a new study).

